Graviton plus vector boson production to NLO in QCD at the LHC

We present the next-to-leading order QCD corrections to the associated production of the vector gauge boson ($Z/W^\pm$) and the graviton in the large extra dimension model at the LHC. We estimate the impact of the QCD corrections on the total cross sections as well as the differential distributions of the gauge bosons and find that they are significant. We also study the dependence of the cross sections on the arbitrary factorization scale and show the reduction in the scale uncertainties at NLO level. Further, we discuss the ultraviolet sensitivity of the theoretical predictions.

==> plotswp.tex <==
\begin{figure}[htb]
\centerline{
\epsfig{file=add.wp.ds.eps,width=15cm,height=12cm,angle=0}}
\caption{Variation of the transverse momentum distribution of $W^+$ boson
with $\delta_s$, keeping the ratio $\delta_s/\delta_c=100$ 
fixed, for $M_s=3$ TeV and $d=4$.}
\label{ds-wp}
\end{figure}
%
\begin{figure}[htb]
\centerline{
\epsfig{file=add.ptmin.wp.d2.eps,width=15cm,height=10cm,angle=0}}
\caption{Total cross section for the associated production of $W^+$ boson and 
the graviton at the LHC, shown as a function of $P_T^{min}$ for $M_s = 3$ TeV 
and $d=2$.}
\label{tot-wp-d2}
\end{figure}
%
\begin{figure}[htb]
\centerline{
\epsfig{file=add.ptmin.wp.d4.eps,width=15cm,height=10cm,angle=0}}
\caption{Total cross section for the associated production of $W^+$ boson and 
the graviton at the LHC, shown as a function of $P_T^{min}$ for $M_s = 3$ TeV 
and $d=4$.}
\label{tot-wp-d4}
\end{figure}
%
\begin{figure}[htb]
\centerline{
\epsfig{file=add.ms.wp.d2.eps,width=15cm,height=10cm,angle=0}}
\caption{Total cross section for the associated production of $W^+$ boson and 
the graviton at the LHC, shown as a function of $M_s$ for $d=2$.}
\label{totms-wp-d2}
\end{figure}
%
\begin{figure}[htb]
\centerline{
\epsfig{file=add.ms.wp.d4.eps,width=15cm,height=10cm,angle=0}}
\caption{Total cross section for the associated production of $W^+$ boson and 
the graviton at the LHC, shown as a function of $M_s$ for $d=4$.}
\label{totms-wp-d4}
\end{figure}
%
\begin{figure}[htb]
\centerline{
\epsfig{file=add.ptmin.wp.kf.eps,width=15cm,height=10cm,angle=0}}
\centerline{
\epsfig{file=add.ms.wp.kf.eps,width=15cm,height=10cm,angle=0}}
\caption{K-factors of the total cross section for the associated production 
of $W^+$ boson and the graviton at the LHC, given as a function of $P_T^{min}$ 
(top) and the scale $M_s$ (bottom).}
\label{tot-wp-kf}
\end{figure}
%
\begin{figure}[htb]
\centerline{
\epsfig{file=add.ptwp.eps,width=8cm,height=9cm,angle=0}}
\caption{Transverse momentum distribution of the $W^+$-boson for $M_s = 3$ 
TeV is shown for different values of the number of extra dimensions $d$.}
\label{pt-wp}
\end{figure}
%
\begin{figure}[htb]
\centerline{
\epsfig{file=add.ptmiss.wp.eps,width=8cm,height=9cm,angle=0}
\epsfig{file=add.ywp.eps,width=8cm,height=9cm,angle=0}}
\caption{Missing transverse momentum distribution of the graviton produced
in association with $W^+$-boson at the LHC, for $M_s = 3$ TeV (left). The
scale uncertainties in the rapidity distribution of $W+$-boson for 
$M_s = 3$ TeV and $d=4$ (right).}
\label{ptmiss-wp}
\end{figure}

